A close-in puffy Neptune with hidden friends: The enigma of TOI 620

We present the validation of a transiting low-density exoplanet orbiting the M2.5 dwarf TOI 620 discovered by the NASA TESS mission. We utilize photometric data from both TESS and ground-based follow-up observations to validate the ephemerides of the 5.09-day transiting signal and vet false positive scenarios. High-contrast imaging data are used to resolve the stellar host and exclude stellar companions at separations $\gtrsim 0.2''$. We obtain follow-up spectroscopy and corresponding precise radial velocities (RVs) with multiple PRV spectrographs to confirm the planetary nature of the transiting exoplanet. We calculate a 5$\sigma$ upper limit of $M_P < 7.1$ M$_\oplus$ and $\rho_P < 0.74$ g cm$^{-3}$, and we identify a non-transiting 17.7-day candidate. We also find evidence for a substellar (1-20 M$_{\rm J}$) companion with a projected separation $\lesssim 20$ au from a combined analysis of Gaia, AO imaging, and RVs. With the discovery of this outer companion, we carry out a detailed exploration of the possibilities that TOI 620 b might instead be a circum-secondary planet or a pair of eclipsing binary stars orbiting the host in a hierarchical triple system. We find, under scrutiny, that we can exclude both of these scenarios from the multi-wavelength transit photometry, thus validating TOI 620 b as a low-density exoplanet transiting the central star in this system. The low density of TOI 620 b makes it one of the most amenable exoplanets for atmospheric characterization, such as with JWST and Ariel, validated or confirmed by the TESS mission to date.

==> rv_table_original.tex <==
% \begin{figure}[htp!]
% \startlongtable
\begin{longrotatetable}
\begin{deluxetable*}{lcccccc}
\label{tab:RVs}
\tablecaption{A full list of the radial velocity values, times, and errors used in this paper.}
\tablehead{\colhead{~~~\bjdtdb [days]} & \colhead{RV [\ms]} & \colhead{Error [\ms]} & \colhead{Instrument} & \colhead{Offset$^\dagger$ [\ms]} & \colhead{Offset Error$^\dagger$ [\ms]}}
\startdata
2458874.042603 \dotfill & -22.034484 \dotfill & 4.963024 \dotfill & iSHELL & -- & -- \\
2458875.075875 \dotfill & -26.544973 \dotfill & 5.031950 \dotfill & iSHELL & -- & -- \\ 
2458895.047871 \dotfill & -32.986091 \dotfill & 4.711785 \dotfill & iSHELL & -- & -- \\
2458897.065268 \dotfill & -24.804451 \dotfill & 11.305265 \dotfill & iSHELL & -- & -- \\
2458899.036716 \dotfill & -13.288003 \dotfill & 4.827823 \dotfill & iSHELL & -- & -- \\
2458900.046926 \dotfill & -24.106087 \dotfill & 5.340227 \dotfill & iSHELL & -- & -- \\ 
2458901.022179 \dotfill & -35.326074 \dotfill & 5.210105 \dotfill & iSHELL & -- & -- \\
2459217.085069 \dotfill & -9.475687 \dotfill & 4.065322 \dotfill & iSHELL & -- & -- \\
2459220.070212 \dotfill & -15.125724 \dotfill & 4.323538 \dotfill & iSHELL & -- & -- \\
2459220.9052352900 \dotfill & -2.323332982814140 \dotfill & 3.950595386632790 \dotfill & NEID & -- & -- \\
2459220.915971710 \dotfill & -13.340735450941500 \dotfill & 3.3149515532090900 \dotfill & NEID & -- & -- \\
2459221.062629 \dotfill & -23.217832 \dotfill & 4.631649 \dotfill & iSHELL & -- & -- \\
2459227.095393 \dotfill & 25.495996 \dotfill & 7.965937 \dotfill & iSHELL & -- & -- \\
2459230.866621630 \dotfill & -6.312635928821160 \dotfill & 1.938692509823220 \dotfill & NEID & -- & -- \\
2459230.877358170 \dotfill & -6.314700031764230 \dotfill & 2.0643178271495100 \dotfill & NEID & -- & -- \\
2459233.027990 \dotfill & -7.535302 \dotfill & 3.890603 \dotfill & iSHELL & -- & -- \\
2459245.996343 \dotfill & -4.819379 \dotfill & 4.869609 \dotfill & iSHELL & -- & -- \\
2459248.5085399998 \dotfill & -35.881376409151443 \dotfill & 17.063194308707494 \dotfill & CARMENES-NIR & -- & -- \\
2459250.5467400001 \dotfill & 8.8157988079908449 \dotfill & 17.999336102091299 \dotfill & CARMENES-NIR & -- & -- \\
2459250.5468000001 \dotfill & -0.89345280980545905 \dotfill & 2.7331968903849844 \dotfill & CARMENES-Vis & -- & -- \\
2459250.939338 \dotfill & -34.967751 \dotfill & 20.550482 \dotfill & iSHELL & -- & -- \\
2459251.765797960 \dotfill & -5.2840423228129 \dotfill & 2.405876788664520 \dotfill & NEID & -- & -- \\
2459251.7765342600 \dotfill & 1.4626090051028100 \dotfill & 2.1969586673225400 \dotfill & NEID & -- & -- \\
2459251.940203 \dotfill & -8.451056 \dotfill & 10.230815 \dotfill & iSHELL & -- & -- \\
2459252.938448 \dotfill & -0.331670 \dotfill & 3.461951 \dotfill & iSHELL & -- & -- \\
2459255.020459 \dotfill & 37.183406 \dotfill & 5.894541 \dotfill & iSHELL & -- & -- \\
2459256.017137 \dotfill & 46.297052 \dotfill & 7.107408 \dotfill & iSHELL & -- & -- \\ 
2459257.009042 \dotfill & 43.079344 \dotfill & 5.833387 \dotfill & iSHELL & -- & -- \\
2459258.011730 \dotfill & 38.230759 \dotfill & 4.895004 \dotfill & iSHELL & -- & -- \\
2459261.040202 \dotfill & 14.988584 \dotfill & 7.516446 \dotfill & iSHELL & -- & -- \\
2459267.742876360 \dotfill & -2.6656154658148200 \dotfill & 3.0919206961484500 \dotfill & NEID & -- & -- \\
2459267.753612430 \dotfill & -2.8207232837875700 \dotfill & 2.539294663668620 \dotfill & NEID & -- & -- \\
2459269.006339 \dotfill & 36.290174 \dotfill & 16.236162 \dotfill & iSHELL & -- & -- \\
2459269.9424637724 \dotfill & -11.465980735247893 \dotfill & 2.5064150319507674 \dotfill & MAROON-X  blue & -1.5 \dotfill & 0.5 \dotfill \\
2459269.9424637724 \dotfill & -11.195024380386242 \dotfill & 1.765484687609815 \dotfill & MAROON-X  red & -2.0 \dotfill & 0.5 \dotfill \\
2459273.024693 \dotfill & 41.528186 \dotfill & 19.956296 \dotfill & iSHELL & -- & -- \\
2459273.4763400001 \dotfill & 0.95482504898741727 \dotfill & 1.6968127526575041 \dotfill & CARMENES-Vis & -- & -- \\
2459273.4764299998 \dotfill & -7.8304032911941306 \dotfill & 7.1968140883213296 \dotfill & CARMENES-NIR & -- & -- \\
2459273.7641193500 \dotfill & 5.9362809130457200 \dotfill & 1.6784596871803700 \dotfill & NEID & -- & -- \\
2459273.774855110 \dotfill & 4.606182098032800 \dotfill & 1.8952827614466200 \dotfill & NEID & -- & -- \\
2459279.744662190 \dotfill & 11.395123857089300 \dotfill & 2.3799394685895700 \dotfill & NEID & -- & -- \\
2459279.7589467200 \dotfill & 6.7617674004103100 \dotfill & 1.9917104863724900 \dotfill & NEID & -- & -- \\
2459299.3345599999 \dotfill & 4.8179084487247019 \dotfill & 1.6743946944978061 \dotfill & CARMENES-Vis & -- & -- \\
2459299.3343600002 \dotfill & 15.118511553049487 \dotfill & 6.6191803954393214 \dotfill & CARMENES-NIR & -- & -- \\
2459300.4146799999 \dotfill & 3.4786951860735087 \dotfill & 6.6240773651457721 \dotfill & CARMENES-NIR & -- & -- \\
2459300.4151699999 \dotfill & -0.67898072025100031 \dotfill & 1.3814786079320489 \dotfill & CARMENES-Vis & -- & -- \\
2459301.3959200000 \dotfill & -1.5129915364868509 \dotfill & 5.4494121726412921 \dotfill & CARMENES-NIR & -- & -- \\
2459301.3960899999 \dotfill & -2.7454809757525540 \dotfill & 1.6613025654761262 \dotfill & CARMENES-Vis & -- & -- \\
2459302.4461599998 \dotfill & -12.043879724468709 \dotfill & 9.7696609586735708 \dotfill & CARMENES-NIR & -- & -- \\
2459302.4463300002 \dotfill & -4.5931016349712559 \dotfill & 2.8141702440924852 \dotfill & CARMENES-Vis & -- & -- \\
2459319.904094 \dotfill & 19.940731 \dotfill & 5.761645 \dotfill & iSHELL & -- & -- \\
2459320.909564 \dotfill & -2.776073 \dotfill & 5.116766 \dotfill & iSHELL & -- & -- \\
2459321.840075911 \dotfill & -5.940675298753413 \dotfill & 1.9343547313481777 \dotfill & MAROON-X  blue & 0.0\dotfill & 0.0\dotfill \\
2459321.840075911 \dotfill & -8.096022192989969 \dotfill & 1.2621461995522072 \dotfill & MAROON-X  red & 0.0\dotfill & 0.0\dotfill \\
2459321.909542 \dotfill & -8.138227 \dotfill & 10.567687 \dotfill & iSHELL & -- & -- \\
2459322.7015060800 \dotfill & -4.731257079614970 \dotfill & 1.993903623518750 \dotfill & NEID & -- & -- \\
2459322.712241580 \dotfill & -0.7338693277052070 \dotfill & 2.1178815233463000 \dotfill & NEID & -- & -- \\
2459322.864615 \dotfill & -22.521940 \dotfill & 4.541347 \dotfill & iSHELL & -- & -- \\
2459328.783324 \dotfill & -27.131826 \dotfill & 5.019038 \dotfill & iSHELL & -- & -- \\
2459331.781398 \dotfill & -21.772759 \dotfill & 5.928742 \dotfill & iSHELL & -- & -- \\
2459333.8101825006 \dotfill & 1.0059787165260885 \dotfill & 1.7057484590994214 \dotfill & MAROON-X  blue & 0.0\dotfill & 0.0\dotfill \\
2459333.8101825006 \dotfill & 2.6643851437448376 \dotfill & 1.0866732999504392 \dotfill & MAROON-X  red & 0.0\dotfill & 0.0\dotfill \\
2459334.7615285106 \dotfill & -1.0779132048128923 \dotfill & 1.934006929331307 \dotfill & MAROON-X  blue & 0.0\dotfill & 0.0\dotfill \\
2459334.7615285106 \dotfill & -1.4607271174950232 \dotfill & 1.284395501322427 \dotfill & MAROON-X  red & 0.0\dotfill & 0.0\dotfill \\
2459352.691481520 \dotfill & 5.861101917380690 \dotfill & 2.4140101347212000 \dotfill & NEID & -- & -- \\
2459352.7022162000 \dotfill & 6.37290697280869 \dotfill & 2.70763855230119 \dotfill & NEID & -- & -- \\
2459361.7652081545 \dotfill & 0.4940627942301865 \dotfill & 1.2859957200992325 \dotfill & MAROON-X  blue & 2.0\dotfill & 1.0\dotfill \\
2459361.7652081545 \dotfill & -3.447412236588432 \dotfill & 0.7951626413400593 \dotfill & MAROON-X  red & 2.5\dotfill & 1.0\dotfill \\
2459362.784009 \dotfill & -12.483647 \dotfill & 10.330877 \dotfill & iSHELL & -- & -- \\
2459362.78422742 \dotfill & 4.275091215196238 \dotfill & 1.7966137616539934 \dotfill & MAROON-X  blue & 2.0\dotfill & 1.0\dotfill \\
2459362.78422742 \dotfill & 4.294219520636129 \dotfill & 0.7391847520663877 \dotfill & MAROON-X  red & 2.5\dotfill & 1.0\dotfill \\
2459363.7391403653 \dotfill & 4.714408696863207 \dotfill & 1.6999607301395838 \dotfill & MAROON-X  blue & 2.0\dotfill & 1.0\dotfill \\
2459363.7391403653 \dotfill & 3.0265388399905127 \dotfill & 0.999853349071746 \dotfill & MAROON-X  red & 2.5\dotfill & 1.0\dotfill \\
2459363.770313 \dotfill & 0.036033 \dotfill & 16.678696 \dotfill & iSHELL & -- & -- \\
2459368.754018193 \dotfill & 4.1113936048769855 \dotfill & 2.1698403568078795 \dotfill & MAROON-X  blue & 2.0\dotfill & 1.0\dotfill \\
2459368.754018193 \dotfill & 0.2448733112044385 \dotfill & 1.0530668019209113 \dotfill & MAROON-X  red & 2.5\dotfill & 1.0\dotfill \\
\enddata
\tablenotetext{\dagger}{See explanation for the offset and offset error in section \ref{sec:primary_analysis}.}

\end{deluxetable*}
\end{longrotatetable}
% \end{figure}
